Measurement of Z/gamma*+jet+X angular distributions in ppbar collisions at sqrt{s}=1.96 TeV

We present the first measurements at a hadron collider of differential cross sections for Z+jet+X production in delta phi(Z, jet), |delta y(Z, jet)| and |y_boost(Z, jet)|. Vector boson production in association with jets is an excellent probe of QCD and constitutes the main background to many small cross section processes, such as associated Higgs production. These measurements are crucial tests of the predictions of perturbative QCD and current event generators, which have varied success in describing the data. Using these measurements as inputs in tuning event generators will increase the experimental sensitivity to rare signals.

==> additional.tex <==
\clearpage
\section{Tables of Results}
Tables \ref{tab:fulldphi25} to \ref{tab:fullyb45} contain the normalised differential cross sections, $1/\sigma\times d\sigma/d X$, for the three angular variables \dphi, \adrap\ and \ayboost. 
For each bin we present the bin edges, bin average (defined in the main text), measured value, statistical uncertainty, uncorrelated systematic uncertainty, and the systematic uncertainties from these sources, which are correlated across all bins and all distributions: 
\begin{enumerate}
\item $\Delta \phi, \Delta y, y_{\text{boost}}$ reweighting uncertainty; 
\item Jet y reweighting uncertainty; 
\item \Z\ p$_{\text{T}}$\ reweighting uncertainty; 
\item Jet p$_{\text{T}}$\ reweighting uncertainty; 
\item Data overlay on simulation uncertainty; 
\item Muon 1/p$_{\text{T}}$\ resolution uncertainty; 
\item Muon identification efficiency uncertainty; 
\item Jet identification efficiency uncertainty;
\item Jet energy resolution uncertainty; 
\item Jet energy scale uncertainty.
\end{enumerate}

\input supplemental.tex
